Data Acquisition: A New Frontier in Data-centric AI

As Machine Learning (ML) systems continue to grow, the demand for relevant and comprehensive datasets becomes imperative. There is limited study on the challenges of data acquisition due to ad-hoc processes and lack of consistent methodologies. We first present an investigation of current data marketplaces, revealing lack of platforms offering detailed information about datasets, transparent pricing, standardized data formats. With the objective of inciting participation from the data-centric AI community, we then introduce the DAM challenge, a benchmark to model the interaction between the data providers and acquirers. The benchmark was released as a part of DataPerf. Our evaluation of the submitted strategies underlines the need for effective data acquisition strategies in ML.

==> _backup.tex <==
\begin{table}[t]
\centering
\begin{tabular}{|c|ccccc|c|}
\toprule
\multirow{2}{*}{Allocation Strategy} & \multicolumn{5}{c}{Market} \\
& market$_1$ & market$_2$ & market$_3$
& market$_4$ & market$_5$ & Mean \\
\midrule
Strategy-RFE & \textbf{74.93} & 76.76 & \textbf{76.72} & 72.54 & 75.30 & 75.25 \\
Strategy-CoISFR & 73.45 & \textbf{76.96} & 73.75 & 76.58 & \textbf{77.11} & 75.57 \\
Strategy-$L_2/L_1$ & 47.39 & 74.95 & 73.35 & 77.16 & 76.31 & 69.83 \\
% Strategy-$L_1$ & 47.39 & 74.95 & 73.35 & 77.16 & 76.31 & 69.83 \\
Strategy-$L_\infty$ & 48.03 & 75.10 & 73.40 & \textbf{77.21} & 76.18 & 69.98 \\
Best-mix-strategy & \textbf{74.93} & \textbf{76.96} &  \textbf{76.72} & \textbf{77.21} & \textbf{77.11} & \textbf{76.59} \\
\bottomrule 
\end{tabular}\vspace{0.5em}
\caption{Summary results for all strategies. Strategy-CoISFR performs the best in general and achieves the highest performance on most data markets. Strategy-$L_p$ is suboptimal on data markets 1-3, though, its performance comes to the top in data market 4 and is also quite close to other strategies in data markets 5. \TODO{Combine all Strategies into one table/figure. Compact representation of strategy-i, maybe one bar with error bars. Rename the algo names to reflect their semantics.}
}
\label{tab:sol123mix}
\end{table}



\begin{table}[t]
\centering
\begin{tabular}{|c|ccccc|c|}
\toprule
\multirow{2}{*}{Allocation Strategy} & \multicolumn{5}{c}{Market} \\
& market$_1$ & market$_2$ & market$_3$
& market$_4$ & market$_5$ & Mean \\
\midrule
Strategy-Single-1 & 75.27 & 71.55 & 72.38 & 74.64 & 72.38 & 73.24 \\
Strategy-Single-2 & 73.21 & 72.14 & 72.14 & 72.02 & 72.14 & 72.33 \\
Strategy-Single-3 & 52.01 & 71.01 & 71.01 & 32.37 & 71.01 & 59.48 \\
Strategy-Single-4 & 71.65 & 56.03 & 75.99 & 46.82 & 75.99 & 65.30 \\
Strategy-Single-5 & 74.49 & 74.95 & 73.72 & 77.43 & 76.05 & 75.33 \\
Strategy-Single-6 & 75.45 & 73.04 & 74.57 & 73.76 & 74.58 & 74.28 \\
Strategy-Single-7 & 73.03 & 70.46 & 72.99 & 74.89 & 72.99 & 72.87 \\
Strategy-Single-8 & 50.50 & 71.14 & 70.10 & 71.77 & 43.60 & 61.42 \\
Strategy-Single-9 & 73.52 & 73.32 & 73.91 & 75.88 & 76.80 & 74.69 \\
Strategy-Single-10 & 74.28 & 73.32 & 78.36 & 76.96 & 76.51 & 75.89 \\
Strategy-Single-11 & 72.24 & 71.58 & 56.19 & 73.96 & 74.75 & 69.74 \\
Strategy-Single-12 & 71.81 & 74.77 & 75.86 & 76.17 & 76.99 & 75.12 \\
Strategy-Single-13 & 70.78 & 72.84 & 76.68 & 74.91 & 75.25 & 74.09 \\
Strategy-Single-14 & 77.63 & 73.88 & 71.73 & 72.51 & 48.08 & 68.77 \\
Strategy-Single-15 & 72.61 & 76.36 & 77.59 & 77.25 & 77.71 & 76.30 \\
Strategy-Single-16 & 75.93 & 77.94 & 76.14 & 74.21 & 75.05 & 75.85 \\
Strategy-Single-17 & 69.27 & 76.59 & 44.26 & 73.21 & 72.79 & 67.22 \\
Strategy-Single-18 & 74.45 & 70.86 & 68.92 & 69.26 & 71.95 & 71.09 \\
Strategy-Single-19 & 49.53 & 74.12 & 74.58 & 74.48 & 53.30 & 65.20 \\
Strategy-Single-20 & 76.48 & 77.02 & 74.48 & 78.06 & 76.21 & \textbf{76.45} \\
Strategy-All & 74.41 & 74.16 & 73.86 & 73.95 & 73.44 & 73.96 \\
Strategy-20\% & 75.56 & 74.38 & 74.85 & 75.04 & 74.97 & 74.96 \\
Strategy-40\% & 75.46 & 73.86 & 75.06 & 74.97 & 75.36 & 74.94 \\
Strategy-60\%& 74.94 & 71.82 & 74.48 & 74.92 & 74.96 & 74.23 \\
Strategy-80\%& 74.10 & 71.05 & 73.96 & 75.07 & 73.01 & 73.44 \\
\bottomrule
\end{tabular}
\caption{\TODO{Name Market 0-4 to 1-5. and add all Strategy-single markets} A summary of the performance of all strategies across the five distinct markets. Notably, \textsf{Strategy-Single-20} and \textsf{Strategy-$20\%$} exhibit superior performance compared to other strategies, with \textsf{Strategy-Single-20} being the top performer, highlighted in bold text. The values represent the official evaluation metric, where higher values indicate better performance. The `Mean' column denotes the mean performance of each strategy across all markets.}
\label{tab:baseline-approaches}
\end{table}


We compare the aforementioned approaches across five distinct markets. For \textsf{Strategy-Single-$i$}, we select the worst, medium, and best performance among the twenty providers. Their provider identifiers are 3, 2, and 20, respectively. For \textsf{Strategy-$p\%$}, we consider the four different levels $p \in \{20, 40, 60, 80\}$. Note that \textsf{Strategy-All} is equivalent to \textsf{Strategy-$0\%$}.

Despite the simplicity of \textsf{Strategy-Single-$i$} approach, \textsf{Strategy-Single-$20$} achieves the best performance with $76.45$. However, it is noteworthy that this approach may not be practical in real-world scenarios as data acquirers typically do not have any information about which provider owns high-quality data without evaluating it. In fact, the same strategy with provider 3, \textsf{Strategy-Single-$3$}, gives the worst performance with $59.48$. Evaluating all providers' data quality is not practically feasible as the number of data providers might be large. Compared to \textsf{Strategy-All}, \textsf{Strategy-$20\%$} shows an improvement by 1\%. However, further exclusion of more providers does not lead to additional improvement. Table~\ref{tab:baseline-approaches} indicates that in each market, only a few outliers have significantly larger distances than the rest. Excluding 20\% of the providers effectively eliminates these outliers. However, excluding more providers beyond this threshold appears to be ineffective, as the distances for the remaining providers do not vary significantly.


